Modelling the nanopore sequencing process with Helicase HMMs

Recent advancements in nanopore sequencing technology, particularly the R10 nanopore from Oxford Nanopore Technology, have necessitated the development of improved data processing methods to utilize their potential for more than 9-mer resolution fully. The processing of the ion currents predominantly utilizes neural network-based methods known for their high basecalling accuracy but face developmental bottlenecks at higher resolutions. In light of this, we introduce the Helicase Hidden Markov Model (HHMM), a novel framework designed to incorporate the dynamics of the helicase motor protein alongside the nucleotide sequence during nanopore sequencing. This model supports the analysis of millions of distinct states, enhancing our understanding of raw ion currents and their alignment with nucleotide sequences. Our findings demonstrate the utility of HHMM not only as a potent visualization tool but also as an effective base for developing advanced basecalling algorithms. This approach offers a promising avenue for leveraging the full capabilities of emerging high-resolution nanopore sequencing technologies.

==> origintext.tex <==
\section{Introduction}
Hidden Markov Models (HMMs) play a crucial role in genome analysis, employed at various stages to model the characteristics of the studied DNA strand. n the preliminary phases encompassing sequencing, assemblies, and mapping, the discrete state space of HMMs effectively represents the measured unit of the DNA strand, known as a \$k\$-mer, denoting consecutive nucleotide bases. ransitioning to later stages, including genome notation, variance detection, and epigenetic inquiries, the state spaces are utilized to characterize functional units of DNA, such as discernible exons and introns. . 

The rapid advancement of large-scale neural networks (NNs) has captivated the attention of genomic scientists, particularly garnering favor within the domain of Nanopore sequencing technologies, owning to their higher sequencing accuracy compared to HMM-based methods. Nanopore sequencing techniques leverage nanometer-scale protein pores to gauge the 'resistance' of a \$k\$-mer on the DNA strand in a singular instance, where \$k\$ corresponds to the depth of the protein pore.  The resistance is reflected in the ion current measured in the protein pore as the DNA strand passes through one base at a time. As the complete DNA strand passes through the pore, a unique sequence of ion currents is measured. Then, a basecaller algorithm is applied to decode the ion current sequence into the nucleotide sequences. 

The idea was drafted in 1980(?), and the first company, Oxford Nanopore Technology (ONT), was established in 2013, as an attempt to commercialise the idea. During the early development, the basecallers were mainly based on a profile HMM model. (ref to profile HMM) Before applying the HMM-based basecaller, typically, a segmentation step is needed to separate events per $k$-mer. The algorithm used for segmentation introduces errors, which would accumulated into the following modelling step with the HMM. To over come the higher error rate, the HMM model needs to be end-to-end. On the other hand, the NN-based method can take in the ion current directly as input and decode the sequence end-to-end, free of segmentation errors. Since 2018, researchers have been devoted to maturing the NN-based basecallers and producing tone of evidence for them to outperform the HMM-based basecallers. In 2019, both the commercial and the research software of the company ONT became NN-based \cite{Wick2019}. 

The NN-based basecaller, however, caused a model mismatch with other methods used in the following stages of the genome analysis. In 2022, the advancing of nanopore sequencing technology has contributed to the success of the first gap-free human genome \cite{2022human}, in which HMM-based analysis tools, named Nanopolish, were used for epigenetic studies. The Nanopolish required separate training on the ion currents due to the insufficiency of knowledge transferring between the NN output and the arbitrary structure of the Nanopolish state space. This extra time- and energy- consuming re-training could be avoided if the basecaller also used an HMM structure. 

Another problem of the NN based basecallers is the adaption to new protein pores with longer depth, which offers higher resolution, i.e. a larger $k$. Along with the advancing of the basecallers is the rapidly involving structure of the protein pores. In the newest R10 protein pore, the measured area is said to be $k=10$, which would be $4^{10}$ classes to classify at a time. This is infeasible for the current NN and GPU to handle, due to which the newest research software Dorado used $k=5$ to compromise. The NN's non-interpretability has also made it hard to embed prior knowledge of the sequencing process \cite{Lokatt}.

We propose an HMM model incorporating the Helicase motor protein behaviour with state space representing $10$-mers. We also demonstrate the training and decoding algorithm to handle such massive state space. We illurstrate the analysis of the ion current signals with the HMM. We also validate the model with basecalling tasks using the human genome data sequenced by ONT R10 material. 

